Feature Preserving and Uniformity-controllable Point Cloud Simplification on Graph

With the development of 3D sensing technologies, point clouds have attracted increasing attention in a variety of applications for 3D object representation, such as autonomous driving, 3D immersive tele-presence and heritage reconstruction. However, it is challenging to process large-scale point clouds in terms of both computation time and storage due to the tremendous amounts of data. Hence, we propose a point cloud simplification algorithm, aiming to strike a balance between preserving sharp features and keeping uniform density during resampling. In particular, leveraging on graph spectral processing, we represent irregular point clouds naturally on graphs, and propose concise formulations of feature preservation and density uniformity based on graph filters. The problem of point cloud simplification is finally formulated as a trade-off between the two factors and efficiently solved by our proposed algorithm. Experimental results demonstrate the superiority of our method, as well as its efficient application in point cloud registration.

==> main/statement.tex <==
We describe point cloud simplification as a process of resampling the point cloud:
given a point cloud $\mathbf{X}$ with $|\mathbf{X}| = N$, find a point cloud $\mathbf{X}' \subset \mathbf{X}$
with $|\mathbf{X}'| = M < N$. The simplification rate is defined as $\alpha = \frac M N$.

A point cloud $\mathbf{X}$ with $N$ points, each of which is composed of $K$ attributes, is represented as
$\mathbf{X} \in \mathbb R^{N \times K}$, where the $i$-th row denoted as $\vec{x}_i ^ {\mathrm{T}}$
represents the $i$-th point.
Attributes can be coordinates, normals, colors, etc., where coordinates are compulsory, i.e., $K \ge 3$.
In order to represent the simplified point cloud, we introduce a resampling diagonal matrix
denoted as $\mathbf{\Psi} \in \mathbb R^{N \times N}$ with $\Psi_{i,i} = 1$
if $\vec{x}_i$ is in the simplified point cloud and $\Psi_{i,i} = 0$ otherwise. 
Thus, the simplified point cloud is represented as $\mathbf{\Psi X}$.

Our goal is to find the optimal resampling matrix $\mathbf{\Psi}$ so as to keep most geometry
features like edges of the point cloud while controlling its evenness. This is essentially a trade-off between  the evenness of points in the simplified point cloud and sharp features, which is formulated in the next section.
